A Formal Model for Programming Wireless Sensor Networks

In this paper we present new developments in the expressiveness and in the theory of a Calculus for Sensor Networks (CSN). We combine a network layer of sensor devices with a local object model to describe sensor devices with state. The resulting calculus is quite small and yet very expressive. We also present a type system and a type invariance result for the calculus. These results provide the fundamental framework for the development of programming languages and run-time environments.

==> fig-reduction.tex <==
\begin{myfigure}
  \begin{gather*}
    \disprule{\RlocalCall}
    {
      \frac{
        M (l_i) = (\vec x_i) P_i
        \qquad
        b \geq \energyIn
      }
      {
        \sensord[\invk \thisk {l_i} {\vec v} \seq P_1 \parp P_2]
        \reduces_F 
        \sensor {P_i \subs {\vec v} {\vec x_i} \seq P_1 \parp P_2} M
        p r {b - \energyIn} 
      }
    }
    \\[\rulespace]
    \disprule{\RnoLocalCall}
    {
      \frac{
        l_i \not \in \dom(M)
%        \qquad
%        b \geq \energyIn
      }
      {
        \sensord[\invk \thisk {l_i} {\vec v} \seq P_1 \parp P_2]
        \reduces_F
        \sensor {\invk \thisk {l_i} {\vec v} \seq P_1 \parp P_2} M
        p r b
% {b - \energyIn} 
      }
    }
    \\[\rulespace] 
    \disprule{\RnetCall}
    {
      \frac{
        \dist (p, p') < r 
        \qquad
        b \geq \energyOut
      }
      {
        \begin{array}{l}
%          \tagsensord[\invk \netk {l_i} {\vec v} \seq P_1 \parp P_2]{N} \parn
        \tagsensord[\invk \netk {l_i} {\vec v} \seq P_1 \parp P_2]{S} \parn
          \sensor{P'}{M'}{p'}{r'}{b'}  
          \reduces_F\\
          \hspace{3cm}
          \tagsensord[\invk \netk {l_i} {\vec v} \seq P_1 \parp P_2]
%          {N \parn \sensor{P' \parp \invk {\thisk} {l_i} {\vec
          {S \parn \sensor{P' \parp \invk {\thisk} {l_i} {\vec
                v}}{M'}{p'}{r'}{b'}}  
        \end{array}
      }
    }
    \\[\rulespace]
    \disprule{\Rrelease}
    {
%      \frac{
%        b \geq \energyOut
%      }
%      {
%        \tagsensord[\invk \netk {l_i} {\vec v} \seq P_1 \parp P_2]{N}
        \tagsensord[\invk \netk {l_i} {\vec v} \seq P_1 \parp P_2]{S}
        \reduces_F
        \sensor {P_1 \parp P_2} M p r {b - \energyOut} \parn S
%        N
%      }
    }
    \\[\rulespace]
%     \disprule{\RlocalCall''}
%     {
%       \frac{
%         l_i \not \in \dom(M)
%       }
%       {
%         \sensord[\invk \thisk {l_i} {\vec v} \seq P_1 \parp P_2] \parn
%         N
%         \reduces 
%         \sensord[P_1 \parp P_2] \parn
%         N
%       }
%     }
%     \\[\rulespace]
    \disprule{\Rinstall}
    {
      \frac{
        b \geq \energyIn
      }
      {
        \sensord[{\installd[M']} \seq P_1 \parp P_2] 
        \reduces_F
        \sensor {P_1 \parp P_2}
                {M \methJoin M'} p r {b - \energyIn}
      }
    }
    \\[\rulespace]
    \disprule{\Rsense}
    {
      \frac{
        b \geq \energyIn
      }
      {
        \sensord[\sensed \seq P_1 \parp P_2] 
        \reduces_F
        \sensor {P \subs {F(p)} x \seq P_1 \parp P_2} M
        p r {b - \energyIn}
      }
    }
    \\[\rulespace]
    \disprule{\Rret}
    {
      \frac{
        b \geq \energyIn
      }
      {
        \sensord[v \seq P_1 \parp P_2] 
        \reduces_F
        \sensor {v \parp P_2} M
        p r {b - \energyIn}
      }
    }
    \\[\rulespace]
%     \disprule{\RsenseDef}
%     {
%       \frac{
%         (p, r_s) \not \downarrow N
%       }
%       {
%         \sensord[\sensed \seq P_1 \parp P_2] \parn
%         N
%         \reduces 
%         \sensord[P \subs {\vec \bottom} {\vec x} \seq P_1 \parp P_2] \parn
%         N
%       }
%     }
%     \\[\rulespace]
%     \disprule{\Rsense''}
%     {
%       \frac{
%         (p, r_s) \not \downarrow N
%       }
%       {
%         \sensord[\sensed \seq P_1 \parp P_2] \parn
%         \Value {\vec v} {p'} \parn
%         N
%         \reduces 
%         \sensord[P_1 \parp P_2] \parn
%         \Value {\vec v} {p'} \parn
%         N
%       }
%     }
%     \\[\rulespace]
    \tag{\Rpar, \Rstructural}
    \frac{
      S_1 \reduces_F S_2
    }
    {
      S \parn S_1 
      \reduces_F
      S \parn S_2
    }
    \qquad
    \frac{
      S_1 \congr S_2 \quad\;\; 
      S_2 \reduces_F S_3 \quad\;\;
      S_3 \congr S_4
    }
    {
      S_1
      \reduces_F 
      S_4
    }
    \\[\rulespace]
    \disprule{\Rnetwork}
    {
      \frac{
        S \reduces_F S'
      }
      {
        S, F 
        \reduces
        S', F
      }
    }
  \end{gather*}
\caption{Reduction semantics for processes and networks.}
\label{fig:reduction-semantics}
\end{myfigure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

